Deuterium-Proton Fusion in an Effective Field Theory Constructed from On-Shell Amplitudes

Big Bang nucleosynthesis (BBN) predicts the primordial deuterium abundance to a precision now limited by the nuclear reactions that burn deuterium. For the simplest of them, proton-deuteron radiative capture, d + p -> \gamma + 3He [d(p,\gamma)3He], the precise LUNA data sit below the ab initio benchmark, and BBN reaction networks split on which to adopt. We develop an effective field theory (EFT) expanding in the finite size of the nuclei, building the amplitude with modern on-shell methods that enumerate every tree-level structure consistent with symmetries without the need for an explicit Lagrangian. A global Bayesian fit to the capture data and nuclear-theory priors returns S(0) = 0.209 +/- 0.008 eV b and traces the offset from the ab initio benchmark to a single natural-sized next-to-leading contact term (t_E1 ~ -0.15, the fractional shift of the electric-dipole amplitude) -- equivalently a ~15% lower effective 3He asymptotic normalization. We estimate the leading EFT truncation errors and identify an elastic d-p observable that would separate them. Our results suggest that amplitude methods enable systematic and complete tree-level construction and matching of EFTs for low-energy nuclear reactions.

==> tikzlibraryfeynmangraphz.code.tex <==
\usetikzlibrary{arrows.meta,bbox,bending,calc,decorations.markings,decorations.pathreplacing,fpu,graphs,patterns.meta,quotes}
% utilities
% stolen from https://tex.stackexchange.com/a/463819
\newcommand{\tikz@fmgz@isnumber}[3]{% \tikz@fmgz@isnumber{<Number>}{<True>}{<False>}
    \begingroup
    \pgfkeys{/pgf/fpu/handlers/invalid number/.code={}}%
    \pgfmathfloatparsenumber{#1}%
    \global\pgfmathfloatgetflagstomacro\pgfmathresult\pgfFloatParseFlag%
    \endgroup
    \ifnum\pgfFloatParseFlag=3%
        #3%
    \else%
        #2%
    \fi%
}
% some private routines
\newcount\c@fmgz@counta
\newcount\c@fmgz@countb
\newif\if@tikz@fmgz@debug
\newcommand{\tikz@fmgz@typeout}[1]{\if@tikz@fmgz@debug
\typeout{#1}\fi}
\def\tikz@fmgz@pgfpoint#1,#2\pgf@stop{\pgfpoint{#1}{#2}}
\def\tikz@fmgz@pgfdist#1,#2;#3,#4\pgf@stop{\pgfmathparse{sqrt((#1-#3)*(#1-#3)+(#2-#4)*(#2-#4))}}
\def\tikz@fmgz@pgfangle#1,#2;#3,#4\pgf@stop{\pgfmathparse{atan2(#4-#2,#3-#1)}}
\newif\if@tikz@fmgz@firstup
\newif\iftikz@fmgz@paralell@curve@has@label
\tikzset{fmg/.style={/tikz/Feynmangraphz/install tikz keys,
	/tikz/graphs/use existing nodes,
	/tikz/Feynmangraphz/.cd,every diagram,#1,/tikz/.cd},
	Feynmangraphz/.cd,
		install tikz keys/.code={
			\tikzset{Gluon/.style={%/pgf/fpu/install only={reciprocal},
				draw,decorate,decoration={fmgz gluon,segment length=5pt,amplitude=6pt},propagator
				},
				gluon/.style={/tikz/draw=none,/tikz/decoration={name=none},postaction={Gluon}},
				Photon/.style={%/pgf/fpu/install only={reciprocal},
					draw,decorate,decoration={fmgz photon,segment length=5pt,amplitude=6pt,#1},propagator
				},
				Photon'/.style={%/pgf/fpu/install only={reciprocal},
					draw,decorate,decoration={fmgz photon',segment length=5pt,amplitude=6pt,#1},propagator
				},
				gauge boson/.style={/pgf/fpu/install only={reciprocal},/tikz/draw=none,/tikz/decoration={name=none},
					postaction={/tikz/Feynmangraphz/segment length=9pt,/tikz/Feynmangraphz/amplitude=1.5pt,wiggles,decorate}},
				photon/.style={/tikz/draw=none,/tikz/decoration={name=none},postaction={Photon={#1}}},
				photon'/.style={/tikz/draw=none,/tikz/decoration={name=none},postaction={Photon'={#1}}},
				vertex/.style={circle,inner sep=0.4ex,outer sep=0pt,fill,node contents={}},
				blob/.style={circle,inner sep=1ex,outer sep=0pt,draw,thick,pattern={Lines[angle=45,distance=2pt]},node contents={}},
				wiggles/.style={decoration={
						markings,
						mark=at position 0 with {\global\tikz@fmgz@n-1\relax
							\pgfmathtruncatemacro{\tikz@fmgz@k}{round((6*\pgfdecoratedpathlength+1*\pgfkeysvalueof{/tikz/Feynmangraphz/segment length})/(6*\pgfkeysvalueof{/tikz/Feynmangraphz/segment length}))}%	
							\pgfmathtruncatemacro{\tikz@fmgz@nn}{6*\tikz@fmgz@k}% number of steps
							\pgfmathsetmacro{\tikz@fmgz@step}{1/\tikz@fmgz@nn}%
							\xdef\tikz@fmgz@step{\tikz@fmgz@step}%
							%\pgfmathsetmacro{\tikz@fmgz@nn}{1/\tikz@fmgz@step}% just for debugging
							\tikz@fmgz@typeout{path length=\pgfdecoratedpathlength, k=\tikz@fmgz@k, step length=\tikz@fmgz@step, expected step number=\tikz@fmgz@nn}},
						mark=between positions 0 and 1 step \tikz@fmgz@step with {
							\global\advance\tikz@fmgz@n1\relax
							%\tikz@fmgz@typeout{\tikz@fmgz@tmp@node-m-\pgfkeysvalueof{/pgf/decoration/mark info/sequence number}}
							\path (0,{\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sqrt(abs(sin(\tikz@fmgz@n*60)))*sign(sin(\tikz@fmgz@n*60))})
								coordinate(\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n);
							},
						mark=at position 1 with {%\global\advance\tikz@fmgz@n1\relax
							%\path (0,0) coordinate(\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n);
							%\path (0,{\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sqrt(abs(sin(\tikz@fmgz@n*60)))*sign(sin(\tikz@fmgz@n*60))})
							%	coordinate(\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n);
							\tikz@fmgz@typeout{wiggles final \the\tikz@fmgz@n}%
					 		\draw[shorten >=-0.2pt,shorten <=-0.2pt,propagator] plot[smooth,variable=\t,samples at={0,...,\the\tikz@fmgz@n}]
					  		(\tikz@fmgz@tmp@node-m-\t);
					 		}
						}
				},
				curly wiggles/.style={decoration={%
						markings,
						mark=at position 0 with {\global\tikz@fmgz@n\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}-1\relax
							\pgfmathtruncatemacro{\tikz@fmgz@k}{round((12*\pgfdecoratedpathlength+1*\pgfkeysvalueof{/tikz/Feynmangraphz/segment length})/(12*\pgfkeysvalueof{/tikz/Feynmangraphz/segment length}))}%	
							\pgfmathtruncatemacro{\tikz@fmgz@nn}{12*\tikz@fmgz@k-2*(\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini})+6}% number of steps
							\pgfmathsetmacro{\tikz@fmgz@step}{1/\tikz@fmgz@nn}%
							\xdef\tikz@fmgz@step{\tikz@fmgz@step}%
							\xdef\tikz@fmgz@correctednexpected{\the\numexpr\tikz@fmgz@nn-10}%
							\tikz@fmgz@typeout{path length=\pgfdecoratedpathlength, k=\tikz@fmgz@k, step length=\tikz@fmgz@step, expected step number=\tikz@fmgz@nn}},
						mark=between positions {3*\tikz@fmgz@step} and {1-3*\tikz@fmgz@step} step \tikz@fmgz@step with {
							\global\advance\tikz@fmgz@n1\relax
							\tikz@fmgz@typeout{curly wiggles step=\the\tikz@fmgz@n}%
							\path ({\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sin(\tikz@fmgz@n*30)},
								{\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*(cos(\tikz@fmgz@n*30)-0.5)})
								coordinate(\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n);
							},
						% mark=at position 0.5 with {%\global\advance\tikz@fmgz@n1\relax
						% 	%\path (0,0) coordinate(\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n);
						% 	%\path (0,{\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sqrt(abs(sin(\tikz@fmgz@n*60)))*sign(sin(\tikz@fmgz@n*60))})
						% 	%	coordinate(\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n);
						% 	\tikz@fmgz@typeout{curly wiggles final n=\the\tikz@fmgz@n}%
					 	% 	\draw[shorten >=-0.2pt,shorten <=-0.2pt,propagator] plot[smooth,variable=\t,samples at={\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini},...,\the\tikz@fmgz@n}]
					 	% 	 (\tikz@fmgz@tmp@node-m-\t);
					 	% 	},
						},	
				},
				draw curly wiggles/.style={
					decoration={%
						show path construction,
						curveto code={%
							\path  (\tikzinputsegmentfirst) coordinate (\tikz@fmgz@tmp@node-m-\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}\relax);
							\ifnum\tikz@fmgz@n>\tikz@fmgz@correctednexpected\relax
								\path (\tikzinputsegmentlast) coordinate 	(\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax);
							 	\draw[%shorten >=-0.2pt,shorten <=-0.2pt,
							 	-,propagator] plot[smooth,variable=\t,			
							 	samples at={\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}\relax,...,\the\numexpr\tikz@fmgz@n\relax}]
					 		  	(\tikz@fmgz@tmp@node-m-\t);
							\else
								\typeout{\the\tikz@fmgz@n<=\tikz@fmgz@correctednexpected}%
							\fi	
							},
						lineto code={%
							\path  (\tikzinputsegmentfirst) coordinate (\tikz@fmgz@tmp@node-m-\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}\relax)
							(\tikzinputsegmentlast) coordinate (\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax);
						 	\draw[shorten >=-0.2pt,shorten <=-0.2pt,-,propagator] plot[smooth,variable=\t,			
							 samples at={\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}\relax,...,\the\numexpr\tikz@fmgz@n\relax}]
							   (\tikz@fmgz@tmp@node-m-\t);
							},
						moveto code={%
							\typeout{moveto\tikzinputsegmentlast}
							\path (\tikzinputsegmentlast) coordinate (\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax);
							\pgfpathmoveto{\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n}{center}}%
							\tikzset{color=blue}
							},			
						closepath code=={%
							\typeout{close path}
							},			
							%}
						% markings,
						% mark=at position 0 with {\tikz@fmgz@typeout{curly wiggles final n=\the\tikz@fmgz@n}%
						% 	\draw[shorten >=-0.2pt,shorten <=-0.2pt,-,propagator] plot[smooth,variable=\t,samples at={\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini},...,\the\tikz@fmgz@n}]
					 	% 	(\tikz@fmgz@tmp@node-m-\t);}
					 	},
					decorate	
				},
				truly dotted/.style={% truly dotted lines (from https://tex.stackexchange.com/a/52856)
    				dash pattern=on 0.01*\pgflinewidth off ##1*\pgflinewidth,
					line cap=round,
    				shorten >/.evaluated=0.5*\pgflinewidth,
					shorten </.evaluated=0.5*\pgflinewidth
					},
    			truly dotted/.default=6,
				complete dashes/.code args={on ##1 off ##2}{% from https://tex.stackexchange.com/a/133357
					\tikz@addoption{%
						\pgfgetpath\tikz@fmgz@currentpath%
						\pgfprocessround{\tikz@fmgz@currentpath}{\tikz@fmgz@currentpath}%
						\pgf@decorate@parsesoftpath{\tikz@fmgz@currentpath}{\tikz@fmgz@currentpath}%
						\let\tikz@fmgz@len\pgf@decorate@totalpathlength
						\pgfmathtruncatemacro{\tikz@fmgz@nn}{round((\tikz@fmgz@len-##1)/(##1+##2))}%
						\pgfmathsetmacro{\tikz@fmgz@r}{##1/##2}%
						\pgfmathsetmacro{\tikz@fmgz@off}{\tikz@fmgz@len/((\tikz@fmgz@nn+1)*\tikz@fmgz@r+\tikz@fmgz@nn)}%
						\pgfmathsetmacro{\tikz@fmgz@on}{\tikz@fmgz@r*\tikz@fmgz@off}%
			%             \pgfmathparse{\pgf@decorate@totalpathlength-#1}\let\tikz@fmgz@rest=\pgfmathresult%
			%             \pgfmathparse{#1+#2}\let\tikz@fmgz@onoff=\pgfmathresult%
			%             \pgfmathparse{max(floor(\tikz@fmgz@rest/\tikz@fmgz@onoff), 1)}\let\tikz@fmgz@nfullonoff=\pgfmathresult%
			%             \pgfmathparse{max((\tikz@fmgz@rest-\tikz@fmgz@onoff*\tikz@fmgz@nfullonoff)/\tikz@fmgz@nfullonoff+#2, #2)}\let\tikz@fmgz@offexpand=\pgfmathresult%
						\pgfsetdash{{\tikz@fmgz@on}{\tikz@fmgz@off}}{0pt}%
						}%
				},
				complete dashes/.default={on \pgfkeysvalueof{/tikz/Feynmangraphz/dash length} off \pgfkeysvalueof{/tikz/Feynmangraphz/gap length}},
				complete dash cycle/.code args={on ##1 off ##2}{% ends with gap, for loops etc.
					\tikz@addoption{%
						\pgfgetpath\tikz@fmgz@currentpath%
						\pgfprocessround{\tikz@fmgz@currentpath}{\tikz@fmgz@currentpath}%
						\pgf@decorate@parsesoftpath{\tikz@fmgz@currentpath}{\tikz@fmgz@currentpath}%
						\let\tikz@fmgz@len\pgf@decorate@totalpathlength
						\pgfmathtruncatemacro{\tikz@fmgz@nn}{round(\tikz@fmgz@len/(##1+##2))}%
						\pgfmathsetmacro{\tikz@fmgz@r}{##1/##2}%
						\pgfmathsetmacro{\tikz@fmgz@off}{\tikz@fmgz@len/(\tikz@fmgz@nn*\tikz@fmgz@r+\tikz@fmgz@nn)}%
						\pgfmathsetmacro{\tikz@fmgz@on}{\tikz@fmgz@off*\tikz@fmgz@r}%
						\pgfsetdash{{\tikz@fmgz@on}{\tikz@fmgz@off}}{0pt}%
						}%
				},
				complete dash cycle/.default={on \pgfkeysvalueof{/tikz/Feynmangraphz/dash length} off \pgfkeysvalueof{/tikz/Feynmangraphz/gap length}},
				cross/.style={minimum size=1em,path picture={
					\draw[propagator] (path picture bounding box.north west) -- (path picture bounding box.south east)
						(path picture bounding box.north east) -- (path picture bounding box.south west);
				}},
				counter/.style={circle,draw,propagator,minimum size=1em,alias=tmp@counter,append after command={
					 (tmp@counter.45) edge[propagator,line cap=butt,shorten >=0.5\pgflinewidth,shorten <=0.5\pgflinewidth] (tmp@counter.225)
					 (tmp@counter.135) edge[propagator,line cap=butt,shorten >=0.5\pgflinewidth,shorten <=0.5\pgflinewidth] (tmp@counter.315)
				}},
				curved arrow/.style={%
					postaction={Feynmangraphz/curved arrow/set values={##1},
						decoration={
							markings,
							mark=at position 0 with {%
						 		\pgfmathsetmacro{\tikz@fmgz@t}{1.1*\pgfkeysvalueof{/tikz/Feynmangraphz/curved arrow/length}/(\pgfdecoratedpathlength)}
								\xdef\tikz@fmgz@t{\tikz@fmgz@t}},
							mark=at position {\pgfkeysvalueof{/tikz/Feynmangraphz/curved arrow/position}-0.5*\tikz@fmgz@t} with {\coordinate(\tikz@fmgz@tmp@node-0);},
							mark=at position {\pgfkeysvalueof{/tikz/Feynmangraphz/curved arrow/position}-\tikz@fmgz@t/6} with {\coordinate(\tikz@fmgz@tmp@node-1);},
							mark=at position {\pgfkeysvalueof{/tikz/Feynmangraphz/curved arrow/position}+\tikz@fmgz@t/6} with {\coordinate(\tikz@fmgz@tmp@node-2);},
							mark=at position {\pgfkeysvalueof{/tikz/Feynmangraphz/curved arrow/position}+0.5*\tikz@fmgz@t} with {\coordinate(\tikz@fmgz@tmp@node-3);
								\draw[/tikz/Feynmangraphz/curved arrow/arrow keys] %[-\pgfkeysvalueof{/tikz/Feynmangraphz/curved arrow/tip}]
						 			let \p0=(\tikz@fmgz@tmp@node-0),\p1=(\tikz@fmgz@tmp@node-3),\p2=(\tikz@fmgz@tmp@node-1),\p3=(\tikz@fmgz@tmp@node-2),
						  			\n1={(-5*\x0 + 2*\x1 + 18*\x2 - 9*\x3)/6},
						 			\n2={(2*\x0 - 5*\x1 - 9*\x2 + 18*\x3)/6},
						 			\n3={(-5*\y0 + 2*\y1 + 18*\y2 - 9*\y3)/6},
									\n4={(2*\y0 - 5*\y1 - 9*\y2 + 18*\y3)/6}
						 			in
						 			(\tikz@fmgz@tmp@node-0) .. controls (\n1,\n3) and (\n2,\n4) .. (\tikz@fmgz@tmp@node-3);
								},
							},
						decorate}
		 		},
		 		parallel curve/.style={%
			 		postaction={Feynmangraphz/parallel curve/set values={##1},
						decorate,
						decoration={%
						markings, 
						mark=at position 0 with {% 
							\pgfmathsetmacro{\tikz@fmgz@t}{\pgfkeysvalueof{/tikz/Feynmangraphz/parallel	curve/length}/(\pgfdecoratedpathlength)} 
							\xdef\tikz@fmgz@t{\tikz@fmgz@t}}, 
						mark=at position {\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/position}-0.5*\tikz@fmgz@t} with 
							{\path (0,\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/distance}) coordinate(\tikz@fmgz@tmp@node-0);}, 
						mark=at position {\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/position}-\tikz@fmgz@t/6} with
							{\path (0,\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/distance}) coordinate(\tikz@fmgz@tmp@node-1);}, 
						mark=at position {\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/position}+\tikz@fmgz@t/6} with 
							{\path (0,\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/distance}) coordinate(\tikz@fmgz@tmp@node-2);}, 
						mark=at position {\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/position}+0.5*\tikz@fmgz@t} with 
							{\path (0,\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/distance}) coordinate(\tikz@fmgz@tmp@node-3); 
					 		 \path (\tikz@fmgz@tmp@node-0) edge[Bezier through={(\tikz@fmgz@tmp@node-1)}{(\tikz@fmgz@tmp@node-2)},
								Feynmangraphz/parallel curve/edge options] (\tikz@fmgz@tmp@node-3);}
						}
					},
		 		},
		 		Bezier through/.style 2 args={to path={
			 		let \p0=(\tikztostart),\p1=(\tikztotarget),\p2=##1,\p3=##2,
				  		\n1={(-5*\x0 + 2*\x1 + 18*\x2 - 9*\x3)/6},
				 		\n2={(2*\x0 - 5*\x1 - 9*\x2 + 18*\x3)/6},
				 		\n3={(-5*\y0 + 2*\y1 + 18*\y2 - 9*\y3)/6},
						\n4={(2*\y0 - 5*\y1 - 9*\y2 + 18*\y3)/6}
				 		in
				 		(\tikztostart) .. controls (\n1,\n3) and (\n2,\n4) .. (\tikztotarget) \tikztonodes
		 		}},
		 		Charged/.tip={Stealth[length=\pgfkeysvalueof{/tikz/Feynmangraphz/charged arrow length},
			 		inset=\pgfkeysvalueof{/tikz/Feynmangraphz/charged arrow inset},
					bend]},
		 		FFlow/.tip={Stealth[length=\pgfkeysvalueof{/tikz/Feynmangraphz/fflow arrow length},
			 		inset=\pgfkeysvalueof{/tikz/Feynmangraphz/fflow arrow inset},
					bend]},
		 		Momentum/.tip={Latex[bend]},
		 		momentum arrow/.style={thin,solid,>=Momentum,->},
		 		momentum/.style={parallel curve={##1,edge options/.append style={momentum arrow,momentum annotations,every edge quotes/.append style={inner sep=3pt},##1}}},
		 		momentum annotations/.style={font=\small},
		 		momentum'/.style={parallel curve={distance/.evaluated={-1*(\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/distance})*1pt/1cm},
			 		##1,
			 		edge options/.append style={momentum arrow,font=\small,every edge quotes/.append style={inner sep=3pt},swap,##1}}},
		 		%momentum/.search also={/tikz/Feynmangraphz/parallel curve/},
		 		propagator/.style={thick,line cap=round},
		 		propagators/.style={/tikz/propagator/.append style={##1}},
		 		fermion/.style={propagator,solid},
		 		scalar/.style={propagator,complete dashes},
		 		charged scalar/.style={scalar,curved arrow={set values={##1}}},
		 		charged antiscalar/.style={scalar,curved arrow={set values={arrow={<-},##1}}},
		 		%clear to path/.code={\tikzset{to path={}}},
		 		charged fermion/.style={fermion,curved arrow={set values={##1}}},
		 		charged antifermion/.style={fermion,curved arrow={set values={arrow={<-},##1}}},
				ghost/.style={propagator,truly dotted,curved arrow={set values={##1}}},
		 		fermion flow/.style={gray,-FFlow},
		 		scalar/.style={propagator,complete dashes},
		 		% charged scalar/.style={scalar,curved arrow=##1},
		 		% charged scalar/.default=0.5,
		 		arc starting at/.style={to path={let \p1=($(\tikztotarget)-(\tikztostart)$),
					\n1={abs((\x1*\x1+\y1*\y1)/(\x1*cos(##1)+\y1*sin(##1))/2)},
					\n2={scalar(Mod(540-atan2(-2*\x1*\y1*cos(##1)+(\x1*\x1-\y1*\y1)*sin(##1),(\x1*\x1-\y1*\y1)*cos(##1)-2*\x1*\y1*sin(##1)),360))},
					\n3={ifthenelse(\n2>##1,\n2,\n2+360)}
			 		in %\pgfextra{\tikz@fmgz@typeout{start=\tikztostart, target=\tikztotarget, arc[start angle=#1,end angle=\n3,radius=\n1]}}
			 		(\tikztostart) arc[start angle=##1,end angle=\n3,radius=\n1] \tikztonodes
		 		}},
		 		arc' starting at/.style={to path={let \p1=($(\tikztotarget)-(\tikztostart)$),
					\n1={abs((\x1*\x1+\y1*\y1)/(\x1*cos(##1)+\y1*sin(##1))/2)},
					\n2={scalar(Mod(540-atan2(-2*\x1*\y1*cos(##1)+(\x1*\x1-\y1*\y1)*sin(##1),(\x1*\x1-\y1*\y1)*cos(##1)-2*\x1*\y1*sin(##1)),360))},
					\n3={ifthenelse(\n2<##1,\n2,\n2-360)}
			 		in %\pgfextra{\tikz@fmgz@typeout{start=\tikztostart, target=\tikztotarget, arc[start angle=##1,end angle=\n3,radius=\n1]}}
			 		(\tikztostart) arc[start angle=##1,end angle=\n3,radius=\n1] \tikztonodes
				}}
			},
		},
		debug/.is if=@tikz@fmgz@debug,
		every diagram/.style={every edge quotes/.append style={inner sep=.6em}},
		every Feynman node/.style={},
		step count/.code={\advance\c@fmgz@counta by1\relax},
		segment length/.initial=5pt,% for wiggles and gluons
		amplitude/.initial=2pt,% for wiggles and gluons
		aspect/.initial=0,% for wiggles and gluons
        dash length/.initial=3pt,% for complete dashes
        gap length/.initial=4pt,% for complete dashes
		first up/.is if=@tikz@fmgz@firstup,
		layout layer/.code={% 
			\advance\c@fmgz@countb by1\relax
			\def\tikz@fmgz@tmpl##1/##2\pgf@nil{%
			 	\def\tikz@fmgz@tmpnodenameandoptions{##1}%
			 	\def\tikz@fmgz@tmpnodecontents{##2}%
			}%
			\def\tikz@fmgz@tmpm[##1]##2\pgf@nil{%
			 	\def\tikz@fmgz@tmpnodename{##2}%
			 	\def\tikz@fmgz@tmpnodeoptions{##1}%
			}%
			\c@fmgz@counta0\relax
			\tikzset{Feynmangraphz/step count/.list={#1}}%
			\tikz@fmgz@typeout{Found list with \the\c@fmgz@counta\space entries.}%
			\ifnum\c@fmgz@countb=1\relax
				\edef\tikz@fmgz@tmpx{0}%
			\else
				\pgfmathsetmacro{\tikz@fmgz@tmpx}{\tikz@fmgz@tmpx+\pgfkeysvalueof{/tikz/Feynmangraphz/hsep}/sqrt(1+abs(\the\c@fmgz@counta-\tikz@fmgz@tmpn))}%
			\fi
			\edef\tikz@fmgz@tmpn{\the\c@fmgz@counta}%
			\def\pgffor@scan{\pgfutil@ifnextchar({\pgffor@scanround}{\pgfutil@ifnextchar[{\pgffor@scansquare}{\pgffor@scanone}}}%
			\def\pgffor@scansquare[##1]##2,{\def\pgffor@value{[##1]##2}\pgffor@scanned}%
			\foreach \tikz@fmgz@tmpa [count=\tikz@fmgz@tmpb] in {#1}
				{\tikz@fmgz@typeout{set up \tikz@fmgz@tmpa, item number=\tikz@fmgz@tmpb}%
				 %\expanded{\noexpand\pgfutil@in@{/}{\tikz@fmgz@tmpa}}% test if, is contained in \tikz@fmgz@tmpa
				 \expandafter\pgfutil@in@\expandafter/\expandafter{\tikz@fmgz@tmpa}\relax
				 \ifpgfutil@in@
					\expandafter\tikz@fmgz@tmpl\tikz@fmgz@tmpa\pgf@nil\relax%
				 \else
					\let\tikz@fmgz@tmpnodenameandoptions\tikz@fmgz@tmpa
					\let\tikz@fmgz@tmpnodecontents\empty
				 \fi
				 \expandafter\pgfutil@in@\expandafter[\expandafter{\tikz@fmgz@tmpnodenameandoptions}\relax
				 \ifpgfutil@in@
					\expandafter\tikz@fmgz@tmpm\tikz@fmgz@tmpnodenameandoptions\pgf@nil\relax%
					%\tikzset{Feynmangraphz/local node options/.style/.expand once=\tikz@fmgz@tmpnodeoptions}%
				 \else
					 \let\tikz@fmgz@tmpnodename\tikz@fmgz@tmpnodenameandoptions%
					 \let\tikz@fmgz@tmpnodeoptions\empty%
					 %\tikzset{Feynmangraphz/local node options/.style={}}%
				 \fi
				 \expanded{\noexpand\pgfutil@in@{\pgfkeysvalueof{/tikz/Feynmangraphz/vertex prefix}}{\tikz@fmgz@tmpnodename}}% test if the vertex prefix is contained in \tikz@fmgz@tmpnodename
				 \ifpgfutil@in@
					\path (\tikz@fmgz@tmpx,
						{(0.5+0.5*\c@fmgz@counta-\tikz@fmgz@tmpb)*\pgfkeysvalueof{/tikz/Feynmangraphz/vsep}})
						node [/tikz/Feynmangraphz/every Feynman node,%Feynmangraphz/local node options,
							style/.expanded=\tikz@fmgz@tmpnodeoptions,name=\tikz@fmgz@tmpnodename,vertex]{\tikz@fmgz@tmpnodecontents};
				 \else
				 	%\pgfmathsetmacro{\mytmp}{(0.5+0.5*\c@fmgz@counta-\tikz@fmgz@tmpb)*\pgfkeysvalueof{/tikz/Feynmangraphz/vsep}}%
				 	%\tikz@fmgz@typeout{(\tikz@fmgz@tmpx,\mytmp), a=\the\c@fmgz@counta, b=\tikz@fmgz@tmpb}%
					\path (\tikz@fmgz@tmpx,
						{(0.5+0.5*\c@fmgz@counta-\tikz@fmgz@tmpb)*\pgfkeysvalueof{/tikz/Feynmangraphz/vsep}})
						node [/tikz/Feynmangraphz/every Feynman node,%Feynmangraphz/local node options,
							style/.expanded=\tikz@fmgz@tmpnodeoptions,
							name=\tikz@fmgz@tmpnodename] {\tikz@fmgz@tmpnodecontents};
				 \fi
				}
		},
		simple layout/.style={%
			/tikz/execute at begin scope={%
				\c@fmgz@counta0\relax
				\tikzset{Feynmangraphz/step count/.list={#1}}%
				\pgfmathsetmacro{\tikz@fmgz@tmpx}{0}%
				\c@fmgz@countb0\relax
				\tikzset{Feynmangraphz/layout layer/.list={#1}}%
			}
		},
		vertex prefix/.initial=v,
		in label/.initial=i,
		out label/.initial=f,
		vsep/.initial=2,
		hsep/.initial=2,
		curved arrow/.cd,
			length/.initial=10pt,
	 		tip/.initial=Charged,
			position/.initial=0.5,
			set values/.code={\tikzset{Feynmangraphz/curved arrow/.cd,#1}},
			arrow keys/.style={>=\pgfkeysvalueof{/tikz/Feynmangraphz/curved arrow/tip},->},
			arrow/.style={/tikz/Feynmangraphz/curved arrow/arrow keys/.append style={#1}},
		/tikz/Feynmangraphz/.cd,
		gluon n ini/.initial={-4},
		gluon pre/.initial=4pt,
		gluon post/.initial=4pt,
	 	charged arrow tip/.initial=Charged,
	 	charged arrow length/.initial=10pt,
	 	charged arrow inset/.initial=2pt,
	 	fflow arrow tip/.initial=FFlow,
	 	fflow arrow length/.initial=5pt,
	 	fflow arrow inset/.initial=1pt,
		temporary node prefix/.store in=\tikz@fmgz@tmp@node,
		temporary node prefix=fmgz@tmp,
		%parallel curve/.search also={/tikz/Feynmangraphz/parallel curve/edge options},
		parallel curve/.unknown/.code={%
    		\let\searchname=\pgfkeyscurrentname%
			\tikz@fmgz@typeout{unknown key in parallel curve: \searchname}
		},
		parallel curve/.cd,
			ignore/.code={},
			length/.initial=20pt,% <- this is not the length of the emerging curve
			distance/.initial=6pt,
			position/.initial=0.5,
			edge node/.forward to=/tikz/Feynmangraphz/parallel curve/ignore,
			edge options/.style={length/.forward to=/tikz/Feynmangraphz/parallel curve/length,
				distance/.forward to=/tikz/Feynmangraphz/parallel curve/distance,
				position/.forward to=/tikz/Feynmangraphz/parallel curve/position,
			},
			edge options+/.style={/tikz/Feynmangraphz/parallel curve/.append style={#1}},
			%edge options/.search also=/tikz/Feynmangraphz/parallel curve/,
			style/.style={},
% 			has label/.is if=tikz@fmgz@paralell@curve@has@label,
% 			label/.code={\tikz@fmgz@typeout{label!}\tikz@fmgz@paralell@curve@has@labeltrue
% 				\def\tikz@fmgz@paralell@curve@label{#1}},
% 			parallel label/.style={midway,font=\tiny,/tikz/Feynmangraphz/parallel curve/distant dependent},
			distant dependent/.code={\ifdim\pgfkeysvalueof{/tikz/Feynmangraphz/parallel curve/distance}>0pt
				\tikzset{allow upside down,below}
			\else
				\tikzset{allow upside down,above}
			\fi},
			has label=false,
			set values/.code={\tikzset{Feynmangraphz/parallel curve/.cd,#1}}
}
\newcount\tikz@fmgz@n
\tikzset{even odd clip/.code={\pgfseteorule},% from https://tex.stackexchange.com/a/538932
	}

% \def\pgfpoint@on@fmgz@gluon#1#2#3{%
% 	\pgf@x=#1\pgfdecorationsegmentamplitude%
% 	\pgf@x=\pgfdecorationsegmentaspect\pgf@x%
% 	\pgf@y=#2\pgfdecorationsegmentamplitude%
% 	\pgf@xa=0.083333333333\pgfdecorationsegmentlength%
% 	\advance\pgf@x by#3\pgf@xa%
% 	%\advance\pgf@x by-\generaloffset pt%
%   }	

\pgfdeclaredecoration{fmgz photon}{initial}{%
	\state{initial}[persistent precomputation={%
			\tikzset{/pgf/fpu/install only={reciprocal}}%
			\global\tikz@fmgz@n0\relax
			\pgfmathtruncatemacro{\tikz@fmgz@nn}{round((\pgfdecoratedpathlength)/\pgfdecorationsegmentlength)}% number of steps
			\ifodd\tikz@fmgz@nn
				\edef\tikz@fmgz@nn{\the\numexpr\tikz@fmgz@nn+1}%
			\fi
			\pgfmathsetmacro{\tikz@fmgz@step}{(\pgfdecoratedpathlength-0.01pt)/\tikz@fmgz@nn}% adjusted segment length
			\pgfdecorationsegmentlength=\tikz@fmgz@step pt%
			\edef\tikz@fmgz@correctednexpected{\the\numexpr\tikz@fmgz@nn-2}%
			\tikz@fmgz@typeout{path length=\pgfdecoratedpathlength, step length=\tikz@fmgz@step, expected step number=\tikz@fmgz@nn}%	
			\pgfmathsetmacro{\tikz@fmgz@r}{0.45*min(\pgfdecorationsegmentlength,\pgfdecorationsegmentamplitude)}%		
			\pgfset{inner sep=0pt,minimum width=\tikz@fmgz@r pt}%
			\tikz@fmgz@typeout{r=\tikz@fmgz@r pt, segment length=\the\pgfdecorationsegmentlength, amplitude=\the\pgfdecorationsegmentamplitude}%
	},width=0pt,next state=wiggle]{%
		% \pgfpathmoveto{\pgfpointdecoratedpathfirst}%
		% \pgfpathmoveto{\pgfpoint{\pgfdecorationsegmentlength}{0pt}}%
		% \pgfinterruptpath
		%   \pgfnode{circle}{center}{}{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{\pgfusepath{stroke}}%
		% \endpgfinterruptpath
	}%
	\state{wiggle}[width=\tikz@fmgz@step pt,switch if less than={\pgfdecorationsegmentlength} to final]{%
		%\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{center}}%
		\global\advance\tikz@fmgz@n1\relax
		%\ifnum\tikz@fmgz@n=1\relax
		\ifodd\tikz@fmgz@n
			\pgfpathcurveto%
				{\pgfpoint{0.25\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{0.75\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{\pgfdecorationsegmentlength}{0pt}}%	
		\else
			\pgfpathcurveto%
				{\pgfpoint{0.25\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{0.75\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{\pgfdecorationsegmentlength}{0pt}}%	
		\fi
    }%
	\state{final}[width=1sp]{%
		%\pgfpathmoveto{\pgfpointshapeborder{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax}{\pgfpointadd{\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax}{center}}{\pgfpoint{-0.4\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}}}%
		%\pgfpathlineto{\pgfpointdecoratedpathlast}%
		%\pgfpathcurveto%
		%		{\pgfpoint{-0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}%
		%		{\pgfpoint{-0.1\pgfdecorationsegmentlength}{0\pgfdecorationsegmentamplitude}}%
		%		{\pgfpointdecoratedpathlast}%
	}%
}	

\pgfdeclaredecoration{fmgz photon'}{initial}{%
	\state{initial}[persistent precomputation={%
			\tikzset{/pgf/fpu/install only={reciprocal}}%
			\global\tikz@fmgz@n0\relax
			\pgfmathtruncatemacro{\tikz@fmgz@nn}{round((\pgfdecoratedpathlength)/\pgfdecorationsegmentlength)}% number of steps
			\ifodd\tikz@fmgz@nn
				\edef\tikz@fmgz@nn{\the\numexpr\tikz@fmgz@nn+1}%
			\fi
			\pgfmathsetmacro{\tikz@fmgz@step}{(\pgfdecoratedpathlength-0.01pt)/\tikz@fmgz@nn}% adjusted segment length
			\pgfdecorationsegmentlength=\tikz@fmgz@step pt%
			\edef\tikz@fmgz@correctednexpected{\the\numexpr\tikz@fmgz@nn-2}%
			\tikz@fmgz@typeout{path length=\pgfdecoratedpathlength, step length=\tikz@fmgz@step, expected step number=\tikz@fmgz@nn}%	
			\pgfmathsetmacro{\tikz@fmgz@r}{0.45*min(\pgfdecorationsegmentlength,\pgfdecorationsegmentamplitude)}%		
			\pgfset{inner sep=0pt,minimum width=\tikz@fmgz@r pt}%
			\tikz@fmgz@typeout{r=\tikz@fmgz@r pt, segment length=\the\pgfdecorationsegmentlength, amplitude=\the\pgfdecorationsegmentamplitude}%
	},width=0pt,next state=wiggle]{%
	}%
	\state{wiggle}[width=\tikz@fmgz@step pt,switch if less than={\pgfdecorationsegmentlength} to final]{%
		\global\advance\tikz@fmgz@n1\relax
		\unless\ifodd\tikz@fmgz@n
			\pgfpathcurveto%
				{\pgfpoint{0.25\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{0.75\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{\pgfdecorationsegmentlength}{0pt}}%	
		\else
			\pgfpathcurveto%
				{\pgfpoint{0.25\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{0.75\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{\pgfdecorationsegmentlength}{0pt}}%	
		\fi
    }%
	\state{final}[width=1sp]{%
	}%
}	

\pgfdeclaredecoration{fmgz gluon}{initial}{%
	\state{initial}[persistent precomputation={%
			\tikzset{/pgf/fpu/install only={reciprocal}}%
			\global\tikz@fmgz@n0\relax
			\pgfmathtruncatemacro{\tikz@fmgz@nn}{round((\pgfdecoratedpathlength-0.95*\pgfdecorationsegmentlength)/\pgfdecorationsegmentlength)}% number of steps
			\pgfmathsetmacro{\tikz@fmgz@step}{(\pgfdecoratedpathlength-0.95*\pgfdecorationsegmentlength-1pt)/\tikz@fmgz@nn}% adjusted segment length
			\pgfdecorationsegmentlength=\tikz@fmgz@step pt%
			\edef\tikz@fmgz@correctednexpected{\the\numexpr\tikz@fmgz@nn-2}%
			\tikz@fmgz@typeout{path length=\pgfdecoratedpathlength, step length=\tikz@fmgz@step, expected step number=\tikz@fmgz@nn}%	
			\pgfmathsetmacro{\tikz@fmgz@r}{0.45*min(\pgfdecorationsegmentlength,\pgfdecorationsegmentamplitude)}%		
			\pgfset{inner sep=0pt,minimum width=\tikz@fmgz@r pt}%
			\tikz@fmgz@typeout{r=\tikz@fmgz@r pt, segment length=\the\pgfdecorationsegmentlength, amplitude=\the\pgfdecorationsegmentamplitude}%
	},width=0.95\pgfdecorationsegmentlength,next state=coil]{%
		% \pgfpathmoveto{\pgfpointdecoratedpathfirst}%
		% \pgfpathmoveto{\pgfpoint{\pgfdecorationsegmentlength}{0pt}}%
		% \pgfinterruptpath
		%   \pgfnode{circle}{center}{}{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{\pgfusepath{stroke}}%
		% \endpgfinterruptpath
	}%
	\state{coil}[width=\tikz@fmgz@step pt,switch if less than={\pgfdecorationsegmentlength} to final]{%
		%\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{center}}%
		\global\advance\tikz@fmgz@n1\relax
		\ifnum\tikz@fmgz@n=1\relax
			\pgfinterruptpath
				\pgfnode{circle}{center}{}{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{}%
			\endpgfinterruptpath
			\pgfpathmoveto{\pgfpointdecoratedpathfirst}%
			\pgfpathcurveto%
				{\pgfpoint{-0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{-0.2\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpointshapeborder{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax}{\pgfpointadd{\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax}{center}}{\pgfpoint{-0.4\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}}}%	
		\else
			\pgfpathmoveto{\pgfpoint{\pgfdecorationsegmentlength}{0pt}}%
			\pgfinterruptpath
			\pgfnode{circle}{center}{}{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{}%
			\endpgfinterruptpath
			%\pgfpathcircle{\pgfpointshapeborder{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n-1\relax}{\pgfpointadd{\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n-1\relax}{center}}{\pgfpoint{0.1\pgfdecorationsegmentlength}{-\pgfdecorationsegmentamplitude}}}}{0.2*\tikz@fmgz@r pt}%
			\pgfpathmoveto{\pgfpointshapeborder{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n-1\relax}{\pgfpointadd{\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n-1\relax}{center}}{\pgfpoint{0.1\pgfdecorationsegmentlength}{-\pgfdecorationsegmentamplitude}}}}%
			\pgfpathcurveto%
				{\pgfpoint{-0.8\pgfdecorationsegmentlength}{-\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{-2\pgfdecorationsegmentlength}{-\pgfdecorationsegmentamplitude}}%
				{\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n-1\relax}{center}}%
			\pgfpathcurveto%
				{\pgfpoint{-0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{-0.2\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpointshapeborder{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax}{\pgfpointadd{\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax}{center}}{\pgfpoint{-0.4\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}}}%			
			\tikz@fmgz@typeout{x=\the\pgf@x, y=\the\pgf@y, r=\tikz@fmgz@r pt, segment length=\the\pgfdecorationsegmentlength, amplitude=\the\pgfdecorationsegmentamplitude}%
		\fi
    }%
	\state{final}[width=1sp]{%
		\pgfpathmoveto{\pgfpointshapeborder{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax}{\pgfpointadd{\pgfpointanchor{\tikz@fmgz@tmp@node-m-\the\numexpr\tikz@fmgz@n\relax}{center}}{\pgfpoint{-0.4\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}}}%
		%\pgfpathlineto{\pgfpointdecoratedpathlast}%
		\pgfpathcurveto%
				{\pgfpoint{-0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}%
				{\pgfpoint{-0.1\pgfdecorationsegmentlength}{0\pgfdecorationsegmentamplitude}}%
				{\pgfpointdecoratedpathlast}%
	}%
}	


% \pgfdeclaredecoration{fmgz gluon}{initial}{%
% 	\state{initial}[width=0pt,next state=mark,persistent precomputation=\tikzset{/pgf/fpu/install only={reciprocal}}] {%
% 		\global\tikz@fmgz@n\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}\relax
% 		\pgfinterruptpath%
% 		  \pgfscope%
% 			\pgfcoordinate{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{\pgfpointdecoratedpathfirst}%
% 			\pgfcoordinate{\tikz@fmgz@tmp@node-m-last}{\pgfpointdecoratedpathlast}%
% 		  \endpgfscope%
% 		\endpgfinterruptpath%
% 		\pgfmathtruncatemacro{\tikz@fmgz@k}{round((12*\pgfdecoratedpathlength+1*\pgfkeysvalueof{/tikz/Feynmangraphz/segment length})/(12*\pgfkeysvalueof{/tikz/Feynmangraphz/segment length}))}%	
% 		\pgfmathtruncatemacro{\tikz@fmgz@nn}{12*\tikz@fmgz@k-2*(\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini})-2}% number of steps
% 		\pgfmathsetmacro{\tikz@fmgz@step}{\pgfdecoratedpathlength/\tikz@fmgz@nn}%
% 		\xdef\tikz@fmgz@step{\tikz@fmgz@step}%
% 		\xdef\tikz@fmgz@correctednexpected{\the\numexpr\tikz@fmgz@nn-2}%
% 		\tikz@fmgz@typeout{path length=\pgfdecoratedpathlength, k=\tikz@fmgz@k, step length=\tikz@fmgz@step, expected step number=\tikz@fmgz@nn}%
% 	}
% 	\state{mark}[width=\tikz@fmgz@step pt,switch if less than={\tikz@fmgz@step} to final]{%
% 		%\ifnum\tikz@fmgz@step>0\relax
% 		\global\advance\tikz@fmgz@n1\relax
% 		\pgfmathtruncatemacro{\tikz@fmgz@itest}{(\tikz@fmgz@n-\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}>4)&&(\tikz@fmgz@correctednexpected-\tikz@fmgz@n>4)}%
% 		\tikz@fmgz@typeout{step \the\tikz@fmgz@n, test=\tikz@fmgz@itest}%
% 		\pgfinterruptpath%
% 		  \pgfscope%
% 		    \ifnum\tikz@fmgz@itest=1\relax
% 				\pgfcoordinate{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{\pgfpoint{\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*(1-0.2*cos(\tikz@fmgz@n*30))*sin(\tikz@fmgz@n*30)}{\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*(cos(\tikz@fmgz@n*30)-0)}}%
% 			\else
% 				\pgfcoordinate{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{\pgfpoint{0pt}{0pt}}%
% 			\fi	
% 		  \endpgfscope%
% 		\endpgfinterruptpath%
% 		%\fi    
% 		}
% 	\state{final}{%
% 		\global\advance\tikz@fmgz@n1\relax
% 		\pgfcoordinate{\tikz@fmgz@tmp@node-m-\the\tikz@fmgz@n}{\pgfpointanchor{\tikz@fmgz@tmp@node-m-last}{center}}%
% 		\draw[%shorten >=-0.2pt,shorten <=-0.2pt,
% 			-,propagator] plot[smooth,variable=\t,			
% 			samples at={\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}\relax,%
% 			\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}+2\relax,
% 			\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini}+3\relax,
% 			...,
% 			%\the\numexpr\tikz@fmgz@n-2\relax,
% 			\the\numexpr\tikz@fmgz@n\relax}] (\tikz@fmgz@tmp@node-m-\t);
% 	   %\draw[red] (\tikz@fmgz@tmp@node-m-\the\numexpr\pgfkeysvalueof{/tikz/Feynmangraphz/gluon n ini})   -- (\tikz@fmgz@tmp@node-m-last); 
% 		%\pgfpathlineto{\pgfpointdecoratedpathlast}
% 	} 
% }	
	
% obsolete or to become obsolete

% the challenge the following approach has is that the nonlinear transformations may lead to very uneven wiggle lengths	
	% 	wiggles/.style={decoration={show path construction,
	% 		moveto code={},
	%     	lineto code={\expanded{\noexpand\tikz@fmgz@pgfdist\tikzinputsegmentfirst;\tikzinputsegmentlast\noexpand\pgf@stop}%
	% 		  \let\tikz@fmgz@len\pgfmathresult
	% 		  \expanded{\noexpand\tikz@fmgz@pgfangle\tikzinputsegmentfirst;\tikzinputsegmentlast\noexpand\pgf@stop}%
	% 		  \let\tikz@fmgz@angle\pgfmathresult
	% 		  \pgfmathtruncatemacro{\tikz@fmgz@nn}{round(\tikz@fmgz@len/\pgfkeysvalueof{/tikz/Feynmangraphz/segment length})}%
	% 		  \pgfmathsetmacro{\tikz@fmgz@segementlength}{\tikz@fmgz@len/\tikz@fmgz@nn/1cm}%
	% 		  \if@tikz@fmgz@firstup
	% 	  		\draw[shift={(\tikzinputsegmentfirst)},rotate=\tikz@fmgz@angle,propagator]
	% 				plot[smooth,variable=\t,domain=0:\tikz@fmgz@nn,samples=12*\tikz@fmgz@nn+1]
	% 				({\tikz@fmgz@segementlength*\t},
	% 				 {\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sqrt(abs(sin(360*\t)))*sign(sin(360*\t))});
	% 			\global\@tikz@fmgz@firstupfalse
	% 		  \else
	% 	  		\draw[shift={(\tikzinputsegmentfirst)},rotate=\tikz@fmgz@angle,propagator]
	% 				plot[smooth,variable=\t,domain=0:\tikz@fmgz@nn,samples=12*\tikz@fmgz@nn+1]
	% 				({\tikz@fmgz@segementlength*\t},
	% 				{-\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sqrt(abs(sin(360*\t)))*sign(sin(360*\t))});
	% 			\global\@tikz@fmgz@firstuptrue
	% 		  \fi
	%     	},
	%     	curveto code={
	% 			%\expanded{\noexpand\tikz@fmgz@pgfdist\tikzinputsegmentfirst;\tikzinputsegmentlast\noexpand\pgf@stop}%
	% 			%\let\tikz@fmgz@len\pgfmathresult
	% 			\pgfmathsetmacro{\tikz@fmgz@len}{\pgfdecoratedpathlength}%
	% 			\tikzset{allow upside down}%
	% 		    \pgfsetcurvilinearbeziercurve
	%     			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentfirst\pgf@stop}%
	%     			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentsupporta\pgf@stop}%
	%     			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentsupportb\pgf@stop}%
	%     			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentlast\pgf@stop}%
	% 		  \pgftransformnonlinear{\pgfpointcurvilinearbezierorthogonal\pgf@x\pgf@y}%
	% 		  \expanded{\noexpand\pgfcurvilineardistancetotime{\tikz@fmgz@len pt}}%
	% 		  \pgfmathsetmacro{\tikz@fmgz@len}{\tikz@fmgz@len/\pgf@x}%
	% 		  %\let\tikz@fmgz@len\pgfdecoratedpathlength
	% 		  \pgfmathtruncatemacro{\tikz@fmgz@nn}{round(\tikz@fmgz@len/\pgfkeysvalueof{/tikz/Feynmangraphz/segment length})}%
	% 		  \pgfmathsetmacro{\tikz@fmgz@segementlength}{\tikz@fmgz@len/\tikz@fmgz@nn/1cm}%
	% 		  \if@tikz@fmgz@firstup
	% 	  		\draw[propagator] plot[smooth,variable=\t,domain=0:\tikz@fmgz@nn,samples=12*\tikz@fmgz@nn+1]
	% 				({\tikz@fmgz@segementlength*\t},
	% 				 {\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sqrt(abs(sin(360*\t)))*sign(sin(360*\t))});
	% 			%\global\@tikz@fmgz@firstupfalse
	% 			%\draw[{Circle}-{Circle},blue] (0,0) -- (\tikz@fmgz@len pt,0);
	% 		  \else
	% 	  		\draw[propagator] plot[smooth,variable=\t,domain=0:\tikz@fmgz@nn,samples=12*\tikz@fmgz@nn+1]
	% 				({\tikz@fmgz@segementlength*\t},
	% 				{-\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sqrt(abs(sin(360*\t)))*sign(sin(360*\t))});
	% 			%\global\@tikz@fmgz@firstuptrue
	% 			%\draw[{Circle}-{Circle},blue] (0,0) -- (\tikz@fmgz@len pt,0);
	% 		  \fi
	%     	},
	%     	closepath code={}
	% 		}
	% 	},
	% 	gluon/.style={decoration={show path construction,
	% 		moveto code={},
	%     	lineto code={\expanded{\noexpand\tikz@fmgz@pgfdist\tikzinputsegmentfirst;\tikzinputsegmentlast\noexpand\pgf@stop}%
	% 		  \let\tikz@fmgz@len\pgfmathresult
	% 		  \expanded{\noexpand\tikz@fmgz@pgfangle\tikzinputsegmentfirst;\tikzinputsegmentlast\noexpand\pgf@stop}%
	% 		  \let\tikz@fmgz@angle\pgfmathresult
	% 		  \pgfmathtruncatemacro{\tikz@fmgz@nn}{round(\tikz@fmgz@len/\pgfkeysvalueof{/tikz/Feynmangraphz/segment length})}%
	% 		  \pgfmathsetmacro{\tikz@fmgz@segementlength}{\tikz@fmgz@len/(\tikz@fmgz@nn+0.5)/1cm}%
	% 		  \if@tikz@fmgz@firstup
	% 	  		\draw[shift={(\tikzinputsegmentfirst)},rotate=\tikz@fmgz@angle,propagator] plot[smooth,variable=\t,domain=0:\tikz@fmgz@nn,samples=12*\tikz@fmgz@nn+1]
	% 				({\tikz@fmgz@segementlength*\t+\tikz@fmgz@segementlength*\pgfkeysvalueof{/tikz/Feynmangraphz/aspect}*(1-cos(360*\t))},
	% 				 {2*\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sin(360*\t)});
	% 		  \else
	% 	  		\draw[shift={(\tikzinputsegmentfirst)},rotate=\tikz@fmgz@angle,propagator] plot[smooth,variable=\t,domain=0:\tikz@fmgz@nn,samples=12*\tikz@fmgz@nn+1]
	% 				({\tikz@fmgz@segementlength*\t+\tikz@fmgz@segementlength*\pgfkeysvalueof{/tikz/Feynmangraphz/aspect}*(1-cos(360*\t))},
	% 				{-2*\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sin(360*\t)});
	% 		  \fi
	%     	},
	%     	curveto code={\expanded{\noexpand\tikz@fmgz@pgfdist\tikzinputsegmentfirst;\tikzinputsegmentlast\noexpand\pgf@stop}%
	% 			\let\tikz@fmgz@len\pgfmathresult
	% 			\path (\tikzinputsegmentfirst) coordinate (tmp);
	% 		  \pgfsetcurvilinearbeziercurve
	%     			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentfirst\pgf@stop}%
	%     			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentsupporta\pgf@stop}%
	%     			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentsupportb\pgf@stop}%
	%     			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentlast\pgf@stop}%
	% 		  \pgftransformnonlinear{\pgfpointcurvilinearbezierorthogonal\pgf@x\pgf@y}%
	% 		  \expanded{\noexpand\pgfcurvilineardistancetotime{\tikz@fmgz@len pt}}%
	% 		  \pgfmathsetmacro{\tikz@fmgz@len}{\tikz@fmgz@len/\pgf@x}%
	% 		  \pgfmathtruncatemacro{\tikz@fmgz@nn}{round(\tikz@fmgz@len/\pgfkeysvalueof{/tikz/Feynmangraphz/segment length})}%
	% 		  \pgfmathsetmacro{\tikz@fmgz@segementlength}{\tikz@fmgz@len/(\tikz@fmgz@nn+0)/1cm}%
	% 		  \if@tikz@fmgz@firstup
	% 	  		\draw[propagator] plot[smooth,variable=\t,domain=0:\tikz@fmgz@nn,samples=12*\tikz@fmgz@nn+1]
	% 				({\tikz@fmgz@segementlength*\t+\tikz@fmgz@segementlength*\pgfkeysvalueof{/tikz/Feynmangraphz/aspect}*(1-cos(360*\t))},
	% 				 {2*\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sin(360*\t)});
	% 		  \else
	% 	  		\draw[propagator] plot[smooth,variable=\t,domain=0:\tikz@fmgz@nn,samples=12*\tikz@fmgz@nn+1]
	% 				({\tikz@fmgz@segementlength*\t+\tikz@fmgz@segementlength*\pgfkeysvalueof{/tikz/Feynmangraphz/aspect}*(1-cos(360*\t))},
	% 				{-2*\pgfkeysvalueof{/tikz/Feynmangraphz/amplitude}*sin(360*\t)});
	% 		  \fi
	%     	},
	%     	closepath code={}
	% 		}
	%     },
	%     complete dashes/.style={decorate,decoration={show path construction,
	%   		moveto code={},
	%       	lineto code={\expanded{\noexpand\tikz@fmgz@pgfdist\tikzinputsegmentfirst;\tikzinputsegmentlast\noexpand\pgf@stop}%
	%   		  \let\tikz@fmgz@len\pgfmathresult
	%   		 %\expanded{\noexpand\tikz@fmgz@pgfangle\tikzinputsegmentfirst;\tikzinputsegmentlast\noexpand\pgf@stop}%
	%   		  %\let\tikz@fmgz@angle\pgfmathresult
	%         \pgfmathtruncatemacro{\tikz@fmgz@nn}{round((\tikz@fmgz@len-\pgfkeysvalueof{/tikz/Feynmangraphz/dash length})/(\pgfkeysvalueof{/tikz/Feynmangraphz/dash length}+\pgfkeysvalueof{/tikz/Feynmangraphz/gap length}))}%
	%         \pgfmathsetmacro{\tikz@fmgz@r}{\pgfkeysvalueof{/tikz/Feynmangraphz/dash length}/\pgfkeysvalueof{/tikz/Feynmangraphz/gap length}}%
	%         \pgfmathsetmacro{\tikz@fmgz@off}{\tikz@fmgz@len/((\tikz@fmgz@nn+1)*\tikz@fmgz@r+\tikz@fmgz@nn)}%
	%         \pgfmathsetmacro{\tikz@fmgz@on}{\tikz@fmgz@r*\tikz@fmgz@off}%
	%   		  %\pgfmathtruncatemacro{\tikz@fmgz@nn}{round(\tikz@fmgz@len/\pgfkeysvalueof{/tikz/Feynmangraphz/segment length})}%
	%   		  %\pgfmathsetmacro{\tikz@fmgz@segementlength}{\tikz@fmgz@len/\tikz@fmgz@nn/1cm}%
	%         \tikz@fmgz@typeout{length=\tikz@fmgz@len, n=\tikz@fmgz@nn, on=\tikz@fmgz@on, off=\tikz@fmgz@off}%
	%   	  	\draw[propagator,dash pattern=on \tikz@fmgz@on pt off \tikz@fmgz@off pt]
	%   				(\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
	%       	},
	%       	curveto code={\expanded{\noexpand\tikz@fmgz@pgfdist\tikzinputsegmentfirst;\tikzinputsegmentlast\noexpand\pgf@stop}%
	%   			\let\tikz@fmgz@len\pgfmathresult
	%   			\tikzset{allow upside down}%
	%   		  \pgfsetcurvilinearbeziercurve
	%       			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentfirst\pgf@stop}%
	%       			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentsupporta\pgf@stop}%
	%       			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentsupportb\pgf@stop}%
	%       			{\expandafter\tikz@fmgz@pgfpoint\tikzinputsegmentlast\pgf@stop}%
	%   		  \pgftransformnonlinear{\pgfpointcurvilinearbezierorthogonal\pgf@x\pgf@y}%
	%   		  \expanded{\noexpand\pgfcurvilineardistancetotime{\tikz@fmgz@len pt}}%
	%   		  \pgfmathsetmacro{\tikz@fmgz@len}{\tikz@fmgz@len/\pgf@x}%
	%         \pgfmathtruncatemacro{\tikz@fmgz@nn}{round((\tikz@fmgz@len-\pgfkeysvalueof{/tikz/Feynmangraphz/dash length})/(\pgfkeysvalueof{/tikz/Feynmangraphz/dash length}+\pgfkeysvalueof{/tikz/Feynmangraphz/gap length}))}%
	%         \pgfmathsetmacro{\tikz@fmgz@r}{\pgfkeysvalueof{/tikz/Feynmangraphz/dash length}/\pgfkeysvalueof{/tikz/Feynmangraphz/gap length}}%
	%         \pgfmathsetmacro{\tikz@fmgz@off}{\tikz@fmgz@len/((\tikz@fmgz@nn+1)*\tikz@fmgz@r+\tikz@fmgz@nn)}%
	%         \pgfmathsetmacro{\tikz@fmgz@on}{\tikz@fmgz@r*\tikz@fmgz@off}%
	%   		  %\pgfmathtruncatemacro{\tikz@fmgz@nn}{round(\tikz@fmgz@len/\pgfkeysvalueof{/tikz/Feynmangraphz/segment length})}%
	%   		  %\pgfmathsetmacro{\tikz@fmgz@segementlength}{\tikz@fmgz@len/\tikz@fmgz@nn/1cm}%
	%         \tikz@fmgz@typeout{length=\tikz@fmgz@len, n=\tikz@fmgz@nn, on=\tikz@fmgz@on, off=\tikz@fmgz@off}%
	%   	  	\draw[propagator,dash pattern=on \tikz@fmgz@on pt off \tikz@fmgz@off pt]
	%   				(0,0) -- (\tikz@fmgz@len pt,0);
	%         },
	%       	closepath code={}
	%   		}
	%     },
	
\tikzset{dot/.style={circle,fill,inner sep=1.5pt},
pics/momentum arrow/.style={code={%
\def\pv##1{\pgfkeysvalueof{/tikz/momentum arrow/##1}}
\tikzset{/tikz/momentum arrow/.cd,#1}
\pgfmathtruncatemacro{\itest}{\pv{d}>0}
\ifnum\itest>0
\draw[momentum arrow/marrow] (-0.5*\pv{l},\pv{d}) -- (0.5*\pv{l},\pv{d})
node[midway,auto]{\pv{m}};
\else
\draw[momentum arrow/marrow] (-0.5*\pv{l},\pv{d}) -- (0.5*\pv{l},\pv{d})
node[midway,auto]{\pv{m}};
\fi
}},
pics/momentum arrow'/.style={code={%
\def\pv##1{\pgfkeysvalueof{/tikz/momentum arrow/##1}}
\tikzset{/tikz/momentum arrow/.cd,#1}
\pgfmathtruncatemacro{\itest}{\pv{d}>0}
\ifnum\itest>0
\draw[momentum arrow/marrow'] (-0.5*\pv{l},\pv{d}) -- (0.5*\pv{l},\pv{d})
node[midway,auto]{\pv{m}};
\else
\draw[momentum arrow/marrow'] (-0.5*\pv{l},\pv{d}) -- (0.5*\pv{l},\pv{d})
node[midway,auto]{\pv{m}};
\fi
}},momentum arrow/.cd,d/.initial=5mm,l/.initial=1cm,
marrow/.style={-latex},marrow'/.style={latex-},m/.initial={}}
\tikzset{pics/fermion flow/.style={code={%
\def\pv##1{\pgfkeysvalueof{/tikz/fermion flow/##1}}
\tikzset{/tikz/fermion flow/.cd,#1}
\pgfmathtruncatemacro{\itest}{\pv{d}>0}
\ifnum\itest>0
\draw[fermion flow/fflow] (-0.5*\pv{l},\pv{d}) -- (0.5*\pv{l},\pv{d})
node[midway,auto]{\pv{m}};
\else
\draw[fermion flow/fflow] (-0.5*\pv{l},\pv{d}) -- (0.5*\pv{l},\pv{d})
node[midway,auto]{\pv{m}};
\fi
}},fermion flow/.cd,d/.initial=-5mm,l/.initial=1cm,
fflow/.style={-{Latex[bend]},gray!50},m/.initial={}}
% \pgfdeclaredecoration{complete sines}{initial}
% {
%     \state{initial}[
%         width=+0pt,
%         next state=sine,
%         persistent precomputation={\pgfmathsetmacro\matchinglength{
%             \pgfdecoratedinputsegmentlength / int(\pgfdecoratedinputsegmentlength/\pgfdecorationsegmentlength)}
%             \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}
%         }] {}
%     \state{sine}[width=\pgfdecorationsegmentlength]{
%         \pgfpathsine{\pgfpoint{0.25\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
%         \pgfpathcosine{\pgfpoint{0.25\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
%         \pgfpathsine{\pgfpoint{0.25\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
%         \pgfpathcosine{\pgfpoint{0.25\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
% }
%     \state{final}{}
% }


\endinput

